Exposing Hidden Interfaces: LLM-Guided Type Inference for Reverse Engineering macOS Private Frameworks

Private macOS frameworks underpin critical services and daemons but remain undocumented and distributed only as stripped binaries, complicating security analysis. We present MOTIF, an agentic framework that integrates tool-augmented analysis with a finetuned large language model specialized for Objective-C type inference. The agent manages runtime metadata extraction, binary inspection, and constraint checking, while the model generates candidate method signatures that are validated and refined into compilable headers. On MOTIF-Bench, a benchmark built from public frameworks with groundtruth headers, MOTIF improves signature recovery from 15% to 86% compared to baseline static analysis tooling, with consistent gains in tool-use correctness and inference stability. Case studies on private frameworks show that reconstructed headers compile, link, and facilitate downstream security research and vulnerability studies. By transforming opaque binaries into analyzable interfaces, MOTIF establishes a scalable foundation for systematic auditing of macOS internals.

==> figures/symbols.tex <==
\begin{table*}[t!]
\scriptsize
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.3}
\caption{Notation summary for Section~\ref{sec:formalization}. Symbols are grouped by conceptual domain (source-level, binary-level, toolchain-level, linting, and optimization) and cover all entities referenced in the iterative type-recovery and SAT\_INFER formulation.}
\begin{tabular}{l l p{11.5cm}}
\toprule
\textbf{Symbol} & \textbf{Domain} & \cellcolor{orange!10}\textbf{Description} \\
\midrule

\rowcolor{catrow}
\multicolumn{3}{l}{\textit{Headers, Grammar, and ASTs}} \\
$\mathcal{H}=\{h_1,\dots,h_m\}$ & Source-Level & Set of Objective-C headers extracted from the Mach-O target. \\
$h_i$ & Source-Level & A specific header file in $\mathcal{H}$. \\
$\mathbb{G}_{\text{ObjC}}$ & Parsing & Context-free grammar used to parse Objective-C headers. \\
$\texttt{AST}_{h_i}$ & Parsing & AST representation produced by $\texttt{Parse}_{\mathbb{G}_{\text{ObjC}}}(h_i)$. \\
$\mathcal{A}=\bigcup_i \texttt{AST}_{h_i}$ & Source-Level & Union of all header ASTs (the header AST corpus). \\
\midrule
\rowcolor{catrow}
\multicolumn{3}{l}{\textit{Ambiguity and Recovery Targets}} \\
$\mathcal{T}_{\text{ambig}}$ & Typing & Finite set of ambiguous types (e.g., \texttt{id}, \texttt{void *}, \texttt{struct \{...\}}). \\
$\mathcal{G}\subset\mathcal{A}$ & Source-Level & Set of underspecified declarations with types from $\mathcal{T}_{\text{ambig}}$. \\
$g_i$ & Source-Level & A specific underspecified declaration targeted for recovery. \\
$p$ & Source-Level & A parameter of $g_i$ used in the ambiguity definition. \\
\midrule
\rowcolor{catrow}
\multicolumn{3}{l}{\textit{Symbol Binding (Binary-Level)}} \\
$s_i\in\mathcal{S}$ & Binary-Level & Symbol name for $g_i$ (mangled ObjC selector) present in the Mach-O. \\
$\texttt{MangledName}(g_i)$ & Toolchain & Mapping from declaration $g_i$ to its mangled selector string. \\
$\texttt{SymTab}(\texttt{MachO})$ & Binary-Level & Mach-O symbol table used to resolve $s_i$. \\
\midrule
\rowcolor{catrow}
\multicolumn{3}{l}{\textit{Inference Context and Prompt Assembly}} \\
$\mathcal{T}_i=(\mathcal{N}_i,\mathcal{I}_i,\mathcal{L}_i)$ & Mixed & Inference context tuple (natural, tool-observable, and linter signals) for $g_i$. \\
$\mathcal{N}_i$ & Source-Level & Natural context: raw declaration text, $s_i$, $(f_i,\ell_i)$, AST-local metadata and comments. \\
$(f_i,\ell_i)$ & Source-Level & File name and line number where $g_i$ is declared. \\
$\mathcal{I}_i$ & Toolchain-Level & Symbolic interface descriptor over tool-accessible observables for $s_i$. \\
$\mathcal{L}_i=\{(m_j,s_j)\}_{j=1}^k$ & Analysis-Level & Severity-stratified linter messages paired with levels $s_j\in\{\texttt{low},\texttt{medium},\texttt{high}\}$. \\
$P_i$ & Inference & Concrete prompt assembled from $\mathcal{T}_i$ for the constrained LLM query. \\
$\hat{g}$ & Inference & Candidate signature used during refinement (and in tool outputs such as \texttt{Yield}$(\hat{g})$). \\
\midrule
\rowcolor{catrow}
\multicolumn{3}{l}{\textit{Toolchain Functions (Observables for $\mathcal{I}_i$)}} \\
$\texttt{Disas}(s_i)$ & Binary Analysis & Returns instruction-level disassembly for symbol $s_i$. \\
$\texttt{Dec}(s_i)$ & Binary Analysis & Produces decompiled pseudocode for symbol $s_i$. \\
$\texttt{HdrRead}(\texttt{AST}_{h_i})$ & Static Analysis & Extracts local typedefs from header AST $\texttt{AST}_{h_i}$. \\
$\texttt{HdrScan}(\texttt{AST}_{\mathcal{H}})$ & Static Analysis & Scans all header ASTs $\mathcal{H}$ for global typedefs. \\
$\texttt{Yield}(\hat{g})$ & Inference & Emits a candidate return-type hypothesis for partial declaration $\hat{g}$. \\
$\texttt{SymAdr}(s_i)$ & Binary Analysis & Retrieves address-level metadata and linkage information for $s_i$. \\
\midrule
\rowcolor{catrow}
\multicolumn{3}{l}{\textit{Linter Semantics and Messages}} \\
$\mathcal{L}:\texttt{Signature}\rightarrow\mathcal{M}$ & Linting & Semantic linter mapping a candidate signature to a multiset of diagnostics. \\
$\texttt{Signature}$ & Typing & Discrete space of fully-specified method signatures. \\
$\mathcal{M}=\{(m_j,s_j)\}$ & Linting & Multiset of linter messages $m_j$ with severities $s_j\in\{\texttt{low},\texttt{medium},\texttt{high}\}$. \\
$m_j$ & Linting & Human-readable diagnostic message produced by the linter. \\
$s_j$ & Linting & Severity level attached to $m_j$ (\texttt{low}/\texttt{medium}/\texttt{high}). \\
\midrule
\rowcolor{catrow}
\multicolumn{3}{l}{\textit{SAT\_INFER (Weighted Partial MaxSAT Objective)}} \\
$\hat{g}\in\texttt{Signature}$ & Inference & Candidate signature evaluated by the linter and the objective. \\
$\hat{g}^*$ & Inference & Optimal signature minimizing soft violations while satisfying all hard constraints. \\
$\mathcal{C}_{\texttt{hard}}$ & Constraints & Set of hard constraints: $\{c_j\in\mathcal{L}(\hat{g})\mid s_j=\texttt{high}\}$. \\
$\mathcal{C}_{\texttt{soft}}$ & Constraints & Set of soft constraints: $\{c_j\in\mathcal{L}(\hat{g})\mid s_j\in\{\texttt{medium},\texttt{low}\}\}$. \\
$c_j$ & Constraints & Boolean predicate over \texttt{Signature} induced by a linter message. \\
$\lambda(s_j)$ & Objective & Cost weight assigned to severities (e.g., $\lambda(\texttt{medium}){=}2$, $\lambda(\texttt{low}){=}1$). \\
$\mathbb{1}[\cdot]$ & Objective & Indicator function used to count violated soft constraints. \\

\bottomrule
\end{tabular}
\label{tab:notation-summary}
\end{table*}
